Graph Products Revisited: Tight Approximation Hardness of Induced Matching, Poset Dimension and More

Graph product is a fundamental tool with rich applications in both graph theory and theoretical computer science. It is usually studied in the form $f(G*H)$ where $G$ and $H$ are graphs, * is a graph product and $f$ is a graph property. For example, if $f$ is the independence number and * is the disjunctive product, then the product is known to be multiplicative: $f(G*H)=f(G)f(H)$. In this paper, we study graph products in the following non-standard form: $f((G\oplus H)*J)$ where $G$, $H$ and $J$ are graphs, $\oplus$ and * are two different graph products and $f$ is a graph property. We show that if $f$ is the induced and semi-induced matching number, then for some products $\oplus$ and *, it is subadditive in the sense that $f((G\oplus H)*J)\leq f(G*J)+f(H*J)$. Moreover, when $f$ is the poset dimension number, it is almost subadditive. As applications of this result (we only need $J=K_2$ here), we obtain tight hardness of approximation for various problems in discrete mathematics and computer science: bipartite induced and semi-induced matching (a.k.a. maximum expanding sequences), poset dimension, maximum feasible subsystem with 0/1 coefficients, unit-demand min-buying and single-minded pricing, donation center location, boxicity, cubicity, threshold dimension and independent packing.

==> missing-apps.tex <==
% \section{Missing Proofs from Section~\ref{sec: applications}.}
% \label{sec:proofs-apps}

%%%%%%%%% Moved to the main paper
%--------------------------------------
% %\subsection{Proof of Lemma~\ref{lem:elbassioni}}
% \restatethm{Lemma}{\ref{lem:elbassioni}}
% {
% $\alpha(G)\leq \induce{\bipp[G]} \leq \induce{\bipm[G]}+\alpha(G)$.
% }
% \begin{proof}

% First, we show the lower bound of $\induce{\bipp[G]}$.
% Let $I \subseteq V(G)$ be a maximum independent set in $G$.
% Clearly, the set of edges $E'=\set{(u,1)(u,2):  u \in I}$ corresponding to $I$
% is an induced matching in $\bip[G]$ since if there is $u, u'\in I$ such that $(u, 1)(u', 2)\in E'$, then $uu'\in E(G)$, contradicting the fact that $I$ is an independent set.
% Thus, $\bip[G]$ has an induced matching of size at least $\alpha(G)$.

% Next, we show the upper bound of $\induce{\bipp[G]}$.
% Consider any induced matching $\mset$ in $\bipp[G]$.
% We may write $\mset=\mset_1\cup \mset_2$, where $\mset_1$ consists of edges that are
% also present in $\bip[G]$ and $\mset_2= \mset \setminus \mset_1$.
% %
% It can be seen that $|\mset_1|\leq\induce{\bip[G]}$ and
% $|\mset_2|\leq\alpha(G)$.
% The latter is because we can obtain an independent set in $G$ by
% choosing each vertex $u$ corresponding to edges $(u,1)(u,2)$ in $\mset_2$.
% Thus, the lemma follows.
% % \qed
% \end{proof}


%Here we provide proofs missing from Section~\ref{sec: applications}.
%Specifically, we give the proofs of Lemma~\ref{lem:elbassioni}, Corollary
%of Lemma~\ref{lem:induce special 1} and
% Lemma~\ref{lem:induce special 2} and also give some examples
% illustrating the proofs.


%------------------- Induced Matching ----------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof of Lemma~\ref{lemma: poset dimension connections}}
% \label{sec:post-dim-proof}
% Now, we define the operator in a slightly different way.
% For each graph
% $G=(V,E)$, the poset $P[G]$ is defined as a two-layered poset
% $(U \cup U', \preceq_G)$.
% The first layer $U$ consists of vertices $\set{u: u\in V(G)}$,
% and $U' = \set{u': u\in V(G)}$.
% For each vertex $u\in V(G)$, there is an arc $uu'$ joining
% $u\in U$ to $u'\in U'$.
% For each edge $uw\in E(G)$, there is an arc $uw'\in E(P[G])$.
% Thus,
% \begin{align*}
% V(P[G]) &= U\cup U' = \set{v: v\in V(G)} \cup \set{v': v\in V(G)}\\
% E(P[G]) &= \set{uu': u\in V(G)} \cup
%            \set{uw':u\in U, v\in U', uw\in E(G)}
% % \end{align*}
%
% The operator $\tilde P$ is defined similarly to $P$ except that we
% erase edges $uu'$ for all $u\in V(G)$.

% Next, we prove the inequality in Lemma~\ref{lemma: poset dimension connections}.

%\subsection{Proof of Lemma~\ref{lem:elbassioni}}
% \restatethm{Lemma}{\ref{lemma: poset dimension connections}}{
% For any graph $G$,
% $\chi(G) \leq \dimension{\bip[G]} \leq \dimension{\bipp[G]} + \chi(G)$
% }

% \begin{proof}
% Recall that $\bipm[G]$ is almost identical to $\bipp[G]$ except that
% $\bipm[G]$ has no edges of the form $(u, 1)(u,2)$ for all $u\in V(G)$.
% %
% We say that a mapping $\psi:\bipp[G] \rightarrow \R$ {\bf hits}
% a vertex $u \in V(G)$ if $\psi((u,1)) > \psi((u,2))$, and
% $\psi((v,1)) \leq \psi((w,2))$ whenever $vw \in E(G)$. In other words, $\psi$ is a linear order that ``reverses'' the direction of edge $(u,1)(u,2) \in \bipp[G]$.

% The following claim was proved by Hegde and Jain in~\cite{HJ07}.
% We restated it here in our terminology. We also provide the proof for completeness.

% \begin{claim}[\cite{HJ07}]
% \label{claim: HJ}
% Let $X \subseteq V(G)$. There is a mapping $\psi$ that hits all
% vertices in $X$ if and only if $X$ is an independent set in $G$.
% \end{claim}
% \begin{proof}
% One direction is easy to see. Suppose $X \subseteq V(G)$ contains $u,v$ such that $uv \in E(G)$, so the function $\psi$ hitting $\set{u,v}$ means that $\psi((u,2)) > \psi((u,1)) \geq \psi((v,2)) > \psi((v,1)) \geq \psi((u,2))$, an obvious contradiction. In short, we cannot expect to have a linear extension of a directed cycle.

% Conversely, assume that $X$ is an independent set. We define function $\psi$ by processing vertices in $X$ in arbitrary order. When vertex $u \in X$ is considered, we set the values $\psi((u,1)) = 2$ and $\psi((u,2)) = 1$. After we finish, we set $\psi((u,1)) = 0$ and $\psi((u,2)) =  3$ for all other vertices $u$'s whose values $\psi$ were undefined. Now notice that the only way to violate the hitting property of $\psi$ is to have $\psi((u,1)) = 2$ and $\psi((v,2)) = 1$ for some $uv \in E(G)$, but this is impossible because $X$ is an independent set.
% % \qed
% \end{proof}


% Now we prove the inequality.

% The lower bound follows immediately from Claim~\ref{claim: HJ}.
% Let $\tilde \phi: V(\bip[G])\rightarrow\R^d$ be a mapping that realizes
% $\bip[G]$.
% For each coordinate $q$, define $\psi_{q}$ as
% $\psi_{q}((u,1)) = \tilde\phi(((u,1))[q]$ and $\psi_{q}((u,2)) = \tilde \phi((u,2))[q]$, i.e. $\psi_{q}$ is function where we project the $q$th
% coordinate of $\tilde \phi$.
% Observe that, for each vertex $u \in V(G)$, there must be some $\psi_{q}$ that
% hits the vertex $u$.
% We argue that there is a valid coloring of $G$ using at most $d$
% colors.
% To see this, construct a coloring as follows.
% For each vertex $u \in V(G)$, assign a color $q$ to $u$, where $q$
% is the first coordinate such that $\psi_{q}$ hits the vertex $u$.
% Claim~\ref{claim: HJ} guarantees that each color class is an
% independent set.
% Thus, the coloring is valid and $\chi(G) \leq d$.

% To prove the upper bound, let $\phi$ be a function that realizes the
% poset $\bipp[G]$.
% Then, for any vertices $u \neq v$ of $G$, we have
% $\phi((u,1))\leq\phi((v,2))$ if and only if $uv \in E(G)$. Then we need to extend $\phi$ into $\tilde \phi$ such that (i) Each vertex $u \in V(G)$ is hit by some coordinate of $\tilde \phi$, and (ii) For any two vertices of the form $(u,i)$ and  $(v,i)$ where $u \neq v$ and $i \in \set{1,2}$, we must have some coordinates $q, q'$ such that $\tilde \phi((u,1))[q] < \tilde \phi((v,1))[q]$ and $\tilde \phi((u,1))[q'] > \tilde \phi((v,1))[q']$. We only need two more coordinates to satisfy (ii). To deal with (i), it suffices to find a collection of functions $\psi_j$ such
% that each vertex $u \in V(G)$ is hit by some $\psi_j$.
% Then $\tilde\phi$ can be defined by concatenating $\phi$ with all the
% mappings $\psi_j$.
% Each such $\psi_j$ can be obtained from Claim~\ref{claim: HJ} by
% defining, for each $j$, $\psi_j$ to be a map that hits all vertices in
% a color class $j$.
% % \qed
% \end{proof}

% \subsection{Proof of Claim~\ref{cor:poset dimension}}
% Note that $\dimension{\vec{K}_2}=1$. By
% Theorem~\ref{theorem:subadditive}, we have that
% %$\dimension{\bipp[G^k]}$ $\leq$
% $\dimension{\bipp[G^{k-1}]}+\chi(G)\dimension{\bipp[G]} +1$ $\leq$
% $\dimension{\bipp[G^{k-2}]}+2\chi(G)\dimension{\bipp[G]} +2$ $\leq
% \ldots$ $\leq$ $\dimension{\bipp[G]}+(k-1)\chi(G)\dimension{\bipp[G]}
% +(k-1)\leq k\chi(G)\dimension{\bipp[G]}+k$.

% \begin{align*} \dimension{\bipp[G^k]} &\leq
% \dimension{\bipp[G^{k-1}]}+\chi(G)\dimension{\bipp[G]} +1\\ &\leq
% \dimension{\bipp[G^{k-2}]}+2\chi(G)\dimension{\bipp[G]} +2\\ &\leq
% \ldots \leq \dimension{\bipp[G]}+(k-1)\chi(G)\dimension{\bipp[G]}
% +(k-1)\\ &\leq k\chi(G)\dimension{\bipp[G]}+k.\quad\quad\quad % \qed
% \end{align*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Next, we prove Corollary~\ref{cor: main for poset dimension}.

% % \subsection{Proof of Corollary \ref{cor: main for poset dimension}}

% \restatethm{Corollary}{\ref{cor: main for poset dimension}}{
% For any positive integer $r$ and any graph $G$, we have
% \[\chi_f(G)^r \leq \dimension{\bip[G^r]} \leq \chi(G)^r + r
% \chi(G) |V(G)|.\]
% }

% \begin{proof}
% To show the lower bound, we apply
% Lemma~\ref{lemma: poset dimension connections}
% and the fact that the lexicographic product satisfies
% $\chi(G\cdot{H}) \geq \chi_f(G) \chi_f(H)$.
% %
% For the upper bound, we first apply the other part of Lemma~\ref{lemma: poset dimension connections} to get
% \[\dimension{\bip[G^r] \leq \chi(G)^r + \dimension{\bipp[G^r]}} +2 \]
% We prove by induction on $r$ that
% $\dimension{\bipp[G^r]} \leq r \chi(G)|V(G)|$.
% The case $r=1$ is trivial.
% For $r >1$, we apply Theorem~\ref{theorem:subadditive}
% and write $\dimension{\bipp[G^r]}$ as
% \begin{align*}
% \dimension{\bipp[G^{r-1} G]} &\leq \dimension{\bipp[G^{r-1}]} +
% \chi(G)\dimension{\bipp[G]}  \\
%  & \leq   (r-1) \chi(G) |V(G)|+\chi(G) |V(G)|\\
%  & \leq r \chi(G) |V(G)|\,.  &\qedhere
% \end{align*}

% \end{proof}


==> missing-product.tex <==
\section{Missing Proofs from Section~\ref{sec: simplified subadditivity}}
\label{sec:missing-simple-ineq}

In this section, we provide proofs missing from
Section~\ref{sec: simplified subadditivity}.
%Specifically, we prove Lemma~\ref{lem:induce special 1} and Lemma~\ref{lem:induce special 2}.


\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MOVED TO MAIN BODY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof from Section~\ref{sec:im-ind}}
\label{sec:proof-im-ind}

\begin{figure*}
\setlength{\fboxsep}{0pt}
\centering{\fbox{\begin{minipage}{\textwidth}
\subfigure[{$G$, $H$, $\bip[G]$ and $\bip[H]$}]{
% \centering{\fbox{\begin{minipage}{\columnwidth}
  \includegraphics[width=0.5\textwidth, clip=true, trim=3cm 8.6cm 6cm 2.5cm]{induce1_2.pdf}
    \label{fig:induce1_2}
% \end{minipage}}}
}
\subfigure[{$\bip[G\vee H]$}]{
% \centering{\fbox{\begin{minipage}{\columnwidth}
  \includegraphics[width=0.4\textwidth, clip=true, trim=6cm 5cm 5cm 4cm]{induce3_2.pdf}
    \label{fig:induce3_2}
% \end{minipage}}}
}
\end{minipage}}}
\caption{Example of graphs $G$, $H$, $\bipm[G]$, $\bipm[H]$ and $\bip[G\vee H]$, as well as super vertices $V_i^x$. Solid edges (in blue) are edges assigned to  $E_G$, and dashed edges (in gray) are edges assigned to $E_H$. }
\end{figure*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof of Lemma~\ref{lem:induce special 1}}

\restatethm{Lemma}{\ref{lem:induce special 1}}{
For any $u\in V(G)$ and $i\in \{1, 2\}$, $V_i^u$ contains an endpoint
of at most one edge in $\mset_G$.
}

%\begin{lemma}
%For any $u\in V(G)$ and $i\in \{1, 2\}$, $V_i^u$ contains an endpoint of at most one edge in $\mset_G$.
%\end{lemma}
%\begin{proof}
\begin{proof}
For the sake of contradiction, assume that there is a vertex $u\in
V(G)$ such that  $V_1^u$ contains two endpoints of two edges in
$\mset_G$, say $(u,a,1)(v,b,2)$ and $(u,a',1)(v',b',2)$.
(The case of $V_2^u$ is proved analogously.)
Since $(u,a,1)(v,b,2)$ is in $E_G$, we have that $uv\in E(G)$ and thus
$(u,1)(v,2)$ is in $E(\bipm[G])$.
This fact then implies that there is an edge between $(u,a',1)$ and
$(v,b,2)$ in $E_G$ as well, contradicting to the fact that $\mset_G$ (and
thus $\mset$) is an induced matching.

\paragraph{Example}
Consider Fig.~\ref{fig:induce3_2} and let's say that $\mset_G$
contains edges $(u, a, 1)(v, b, 2)$ and $(u, b, 1)(v, a, 2)$ which
means that $V_1^u$ contains endpoints of two edges in
$\mset_G$. Having the first edge in $E_G$ means that $uv\in E(G)$ and
thus $(u, 1), (v, 2)$ is in $E(\bipm[G])$ (as witnessed in
Fig.~\ref{fig:induce1_2}). But then it means
that edge $(u, a, 1)(v, a, 2)$ must be in $E_G$ as well, making
$\mset_G$ (and thus $\mset$) not an induced matching.
\end{proof}



% \subsection{Proof of Lemma~\ref{lem:induce special 2}}

%The next step is to show that in the unified graph, not only the matching $\mset_G$ remains a matching, but it is in fact an induced matching. It follows from this lemma.

% \begin{lemma}\label{lem:induce special 2}
% For any $u, u', v, v'\in V(G)$, if $\mset_G$ contains an edge between vertices in $V_1^u$ and $V_2^v$ and an edge between vertices in $V_1^{u'}$ and $V_2^{v'}$ then there is no edge between vertices in $V_1^u$ and $V_2^{v'}$ in $E_G$.
% \end{lemma}

\restatethm{Lemma}{\ref{lem:induce special 2}}{
For any $u, u', v, v'\in V(G)$, if $\mset_G$ contains an edge between
vertices in $V_1^u$ and $V_2^v$ and an edge between vertices in
$V_1^{u'}$ and $V_2^{v'}$ then there is no edge between vertices in
$V_1^u$ and $V_2^{v'}$ in $E_G$.
}

\begin{proof}
Assume for a contradiction that $\mset_G$ contains edges $(u, a, 1)(v, b, 2)$ and $(u', a', 1)(v', b', 2)$ and there is an edge, say $(u, c, 1)(v', d', 1)$ in $E(G)$.
% Having the last edge in $E_G$ implies that $uv'\in E(G)$ which means that $(u, 1)(v', 2)\in E(\bipm[G])$ which then implies that $(u, a, 1)(v', b', 2)$ is in $E_G$.
Since the edge $(u, c, 1)(v', d', 1)$\bundit{the word ``last edge'' is not clear, so I re-phrase. The old one is ``Having the last edge in $E_G$ implies that $uv'\in E(G)$ which means that $(u, 1)(v', 2)\in E(\bipm[G])$ which then implies that $(u, a, 1)(v', b', 2)$ is in $E_G$.''}
 is in $E_G$, we have $uv'\in{E(G)}$ and thus $(u, 1)(v', 2)\in E(\bipm[G])$.
This implies that $(u, a, 1)(v', b', 2)$ is in $E_G$.
%
This contradicts the fact that $\mset$ is an induced matching in $\bipm[G\vee H]$.

\paragraph{Example} Consider Fig.~\ref{fig:induce3_2}, and let's say
that matching $\mset_G$ contains $(v, a, 1)(u, a, 2)$ and $(u, a,
1)(w, a, 2)$ and there is an edge $(v, b, 1)(w, b, 2)$ which prevents
$\mset_G$ from being an induced matching in the graph of super
vertices. Having the last edge in $E_G$ implies that $(v, 1)(w, 2)\in
E(\bipm[G])$ which in turns implies that $(v, a, 1)(w, a, 2)\in E_G$,
making $\mset_G$ (and thus $\mset$) not an induced matching in
$\bipm[G\vee H]$.
\end{proof}

\end{comment}


\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MOVED TO MAIN BODY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof from Section~\ref{sec:poset-ineq}}
\label{sec:proofs-poset-ineq}

% Next, we prove Lemma~\ref{lem:phi realizes B}.
%\subsection{Proof of Lemma~\ref{lem:phi realizes B}}
%\danupon{I haven't looked at this section yet}


\begin{figure*}
\setlength{\fboxsep}{0pt}
\centering{\fbox{\begin{minipage}{\textwidth}
\subfigure[$\varphi_1$ (cf. Section~\ref{sec: simplified subadditivity}) introduces ``undesirable edges'' such as the bold edge in this picture.]{
  \includegraphics[height=0.22\textheight, clip=true, trim=5cm 6cm 3cm 1cm]{dimension4.pdf}
    \label{fig:dimension4}
}
\subfigure[$\varphi_2$ (cf. Section~\ref{sec: simplified subadditivity}) removes ``desirable edges'' such as the bold edge in this picture.]{
  \includegraphics[height=0.22\textheight, clip=true, trim=3cm 6cm 2cm 1cm]{dimension5.pdf}
    \label{fig:dimension5}
}
\end{minipage}}}
\caption{ }\label{fig:dimension_45}
\end{figure*}



%\begin{figure}
%\subfigure[$\varphi_3$ (cf. Section~\ref{sec: simplified subadditivity}) does not remove any desirable edges and does not introduce some undesirable edges introduced by $\varphi_1$ (e.g., the dashed bold edge in this picture). However, it still introduces some undesirable edge (e.g., the solid bold edge in this picture).]{
%  \includegraphics[height=0.2\textheight, clip=true, trim=3cm 6cm 2cm 1cm]{dimension6.pdf}
%    \label{fig:dimension6}
%}
%\subfigure[$\varphi=\varphi_4$ (cf. Section~\ref{sec: simplified subadditivity}) which realizes {$\bipp[G\cdot H]$}.]{
%  \includegraphics[height=0.2\textheight, clip=true, trim=2cm 6cm 0cm 1cm]{dimension7.pdf}
%    \label{fig:dimension7}
%}
%\caption{}\label{fig:dimension_67}
%\end{figure}


\begin{figure*}
\setlength{\fboxsep}{0pt}
\centering{\fbox{\begin{minipage}{\textwidth}
\begin{center}
 \includegraphics[height=0.3\textheight, clip=true, trim=2cm 6cm 0cm 1cm]{dimension7.pdf}
\end{center}
\end{minipage}}}
\caption{$\varphi_3$ (cf. Section~\ref{sec: simplified subadditivity}) which realizes {$\bipp[G\cdot H]$}.}\label{fig:dimension_67}\label{fig:dimension7}
\end{figure*}


\restatethm{Lemma}{\ref{lem:phi realizes B}}{
$\varphi$ realizes $\bipp[G\cdot H]$.
}
\begin{proof}




We will be using the following properties:

\renewcommand{\theenumi}{P\arabic{enumi}}
%\begin{enumerate}
\squishnum
\item \label{property: embedding of G} For any $(u,1), (v,2) \in
  V(\bipp[G])$,
 $(u,1)(v,2) \in E(\bipp[G])$ $\iff$ $\phi_1((u,1)) < \phi_1((v,2))$.

\item \label{property: embedding of H} For any
  $(a,1)(b,2)\in{V(\bipp[H])}$,
  $(a,1)(b,2) \in E(\bipp[H])$ $\iff$ $\phi_2((a,1)) < \phi_2((b,2))$.

\item \label{property: coloring of G} For any $uv \in E(G)$, $\cset(u) \neq \cset(v)$.
%\end{enumerate}
\squishnumend
\renewcommand{\theenumi}{\arabic{enumi}}



We argue that for any vertices $(u,a,1),(v,b,2) \in V(\bipp[G\cdot H])$,
we have $(u,a,1)(v,b,2) \in E(\bipp[G\cdot H])$ if and only if
$\phi((u,a,1))< \phi((v,b,2))$. We analyze five possible cases.

\begin{itemize}
  \item {\bf Case 1. $u \neq v$ and $uv \in E(G)$:}
    We will show that $\phi((u,a,1))\leq\phi((v,b,2))$.
    First, $(u,a,1)(v,b,2) \in E(\bipp[G\cdot H])$ by construction, and
    $\mathcal{C}(u)\neq\mathcal{C}(v)$ by
    Property~\ref{property: coloring of G}.
    Next, consider the blocks $\bset_0$, $\bset_{\mathcal{C}(u)}$ and
    $\bset_{\mathcal{C}(v)}$. We have
    \squishlist
    \item $\phi((u,a,1))|_{\bset_0} =  \phi_1((u,1)) <
      \phi_1((v,2))=\phi((v,b,2))|_{\bset_0}$ because of
    Property~\ref{property: embedding of G} and
    $(u,1)(v,2)\in{E(\bipp[G])}$.
    \item $\phi((u,a,1))|_{\bset_{\cset(u)}}= \phi_2((a,1)) <  \infty
      = \phi((v,b,2))|_{\bset(\cset(u))}$.
    \item $\phi((u,a,1))|_{\bset_{\cset(v)}}=0 <
           \phi_2((v,2))=\phi((v,b,2))|_{\bset_{\cset(v)}}$.
    \squishend
    This proves the claim.



  \item {\bf Case 2. $u \neq v$ and $uv \not\in E(G)$:}
    We will show that $\phi((u,a,1)) \not< \phi((v,b,2))$.
    First, $(u,a,1)(v,b,2) \not\in E(\bipp[G \cdot H])$ by construction.
    Consider the block $\bset_0$.
    Because of Property~\ref{property: embedding of G} and
    $(u,1) (v,2) \not\in E(\bipp[G])$, we have
    $\phi((u,a,1))|_{\bset_0} =
     \phi_1((u,1))\not < \phi_1((v,2)) = \phi((v,b,2))|_{\bset_0}$.
     Thus, $\phi((u,a,1)) \not< \phi((v,b,2))$.


  \item {\bf Case 3. $u =v$, $a\neq b$ and $ab \in E(H)$: }
   We will show that $\phi((u,a,1)) \leq \phi((v,b,2))$.
   First, $(u,a,1) (v,b,2) \in E(\bipp[G \cdot H])$ by construction.
    Consider each block. We have
    \squishlist
    \item $\phi((u,a,1))|_{\bset_0} = \phi_1((u,1))
                                  = \phi_1((v,2))
                                  = \phi((v,b,2))|_{\bset_0}$.
    \item $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1))
                                   < \phi_2((b,2))
                                   =
                                   \phi((v,b,2))|_{\bset_{\cset(v)}}$
    because $(a,1) (b,2) \in E(\bipp[H])$ and
    Property~\ref{property: embedding of H}.
    \item $\phi((u,a,1))|_{\bset_{\ell}} = 0 \leq \infty
                                      = \phi((v,b,2))|_{\bset_{\ell}}$
          for other blocks $\bset_{\ell}$.
    \squishend
    This proves the claim.

    % In this case, we have $(u,a,1) (v,b,2) \in E(\bipp[G \cdot H])$.
    % In the block $\bset_0$, we have $\phi((u,a,1))|_{\bset_0} = \phi_1((u,1)) = \phi_1((v,2)) =\phi((v,b,2))|_{\bset_0}$, and in
    % the block $\bset_{\mathcal{C}(u)}$ we have
    % $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1))< \phi_2((b,2)) = \phi((v,b,2))|_{\bset_{\cset(v)}}$ due to the fact that $(a,1) (b,2) \in E(\bipp[H])$ and Property~\ref{property: embedding of H}.
    % For other blocks $\bset_l$, we only compare $0$ to $\infty$, that is, $\phi((u,a,1))|_{\bset_l} = 0 \leq \infty = \phi((v,b,2))|_{\bset_l}$.


  \item {\bf Case 4. $u=v$, $a\neq b$ and $ab \not\in E(H)$:}
    We will show that $\phi((u,a,1)) \not< \phi((v,b,2))$.
    First, $(u,a,1) (v,b,2) \not\in E(\bipp[G\cdot H])$ by construction.
    Consider the block $\bset_{\mathcal{C}(u)}$.
    By Property~\ref{property: embedding of H},
    $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1)) \not<
    \phi_2((b,2)) = \phi((v,b,2))|_{\bset_{\cset(v)}}$ , thus proving the claim.



    % Then we have $(u,a,1) (v,b,2) \not\in E(\bipp[G\cdot H])$.
    % In the block $\bset_{\mathcal{C}(u)}$, we have
    % $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1)) \not< \phi_2((b,2)) = \phi((v,b,2))|_{\bset_{\cset(v)}}$, from Property~\ref{property: embedding of H}, implying that $\phi((u,a,1)) \not< \phi((v,b,2))$.


  \item {\bf Case 5. $u=v$ and $a=b$:}
  We will show that $\phi((u,a,1))< \phi((v,b,2))$.
  First, by the definition of the operator $\bipp$,
  $(u,a,1)(v,b,2) \in E(\bipp[G \cdot H])$.
  Next, consider each block.
  \squishlist
  \item $\phi((u,a,1))|_{\bset_0} = \phi_1((u,1)) <
         \phi_1((v,2)) = \phi((v,b,2))|_{\bset_0}$.
  \item $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1)) <
         \phi_2((b,2))= \phi((v,b,2))|_{\bset_{\cset(v)}}$
         by property~\ref{property: embedding of H}.
  \squishend
  This proves the claim.
    % In this case, by the definition of the operator $\bipp$, we have
    % $(u,a,1)(v,b,2) \in E(\bipp[G \cdot H])$.
    % In the block $\bset_0$, we have $\phi((u,a,1))|_{\bset_0} = \phi_1((u,1)) < \phi_1((v,2)) = \phi((v,b,2))|_{\bset_0}$, and in
    % the block $\bset_{\mathcal{C}(u)}$, we have
    % $\phi((u,a,1))|_{\bset_{\cset(u)}} = \phi_2((a,1)) < \phi_2((b,2))= \phi((v,b,2))|_{\bset_{\cset(v)}}$, due to property~\ref{property: embedding of H}. Therefore, it must be the case that
    % $\phi((u,a,1))< \phi((v,b,2))$.
\end{itemize}
%\squishend

\end{proof} 

\end{comment}
